The Moral Debater: A Study on the Computational Generation of Morally Framed Arguments

An audience's prior beliefs and morals are strong indicators of how likely they will be affected by a given argument. Utilizing such knowledge can help focus on shared values to bring disagreeing parties towards agreement. In argumentation technology, however, this is barely exploited so far. This paper studies the feasibility of automatically generating morally framed arguments as well as their effect on different audiences. Following the moral foundation theory, we propose a system that effectively generates arguments focusing on different morals. In an in-depth user study, we ask liberals and conservatives to evaluate the impact of these arguments. Our results suggest that, particularly when prior beliefs are challenged, an audience becomes more affected by morally framed arguments.

==> table-manual-eval-detailed-results-cons.tex <==
\begin{table}[t!]%
	\centering%
	\small
	\renewcommand{\arraystretch}{1}
	\setlength{\tabcolsep}{3pt}%
	\begin{tabular}{lcccc}
		\toprule
		\bf Morals 		& \bf Stance    & \bf Rank 1 & \bf Rank 2  & \bf Rank 3 \\
		\midrule
		Binding   		& Support	&  25\% &  21\%  &  54\%\\
	    Individualizing & Support   &  50\% &  29\%  &  21\%\\
		Uncontrolled	& Support   &  25\% &  50\%  &  25\%\\
		\midrule
		Binding   		& Contest	&  17\% &  21\%  &  62\%\\
		Individualizing & Contest   &  50\% &  46\%  &  4\%\\
		Uncontrolled	& Contest   &  33\% &  33\%  &  33\%\\
		\bottomrule
	\end{tabular}%
	\caption{Considering Conservatives evaluations, this table shows percentage of cases each argument type (binding, individualizing, and uncontrolled) achieved for each rank, considering whether arguments contest or support the user who rated it.}
	\label{manual-main-eval-table-conservatives}%
\end{table}

==> table-manual-eval-detailed-results-lib.tex <==
\begin{table}[t!]%
	\centering%
	\small
	\renewcommand{\arraystretch}{1}
	\setlength{\tabcolsep}{3pt}%
	\begin{tabular}{lcccc}
		\toprule
		\bf Morals 		& \bf Stance    & \bf Rank 1 & \bf Rank 2  & \bf Rank 3 \\
		\midrule
		Binding   		& Support	&  30\% &  35\%  &  35\%\\
	    Individualizing & Support   &  30\% &  40\%  &  30\%\\
		Uncontrolled	& Support   &  40\% &  25\%  &  35\%\\
		\midrule
		Binding   		& Contest	&  30\% &  45\%  &  25\%\\
		Individualizing & Contest   &  45\% &  25\%  &  30\%\\
		Uncontrolled	& Contest   &  25\% &  30\%  &  45\%\\
		\bottomrule
	\end{tabular}%
	\caption{Percentage of cases each argument type (binding, individualizing, and general) achieved for each rank, considering the majority rank.}
	\label{manual-main-eval-table-liberals}%
\end{table}
